Degreewidth: a New Parameter for Solving Problems on Tournaments

In the paper, we define a new parameter for tournaments called degreewidth which can be seen as a measure of how far is the tournament from being acyclic. The degreewidth of a tournament $T$ denoted by $\Delta(T)$ is the minimum value $k$ for which we can find an ordering $\langle v_1, \dots, v_n \rangle$ of the vertices of $T$ such that every vertex is incident to at most $k$ backward arcs (\textit{i.e.} an arc $(v_i,v_j)$ such that $j<i$). Thus, a tournament is acyclic if and only if its degreewidth is zero. Additionally, the class of sparse tournaments defined by Bessy et al. [ESA 2017] is exactly the class of tournaments with degreewidth one. We first study computational complexity of finding degreewidth. Namely, we show it is NP-hard and complement this result with a $3$-approximation algorithm. We also provide a cubic algorithm to decide if a tournament is sparse. Finally, we study classical graph problems \textsc{Dominating Set} and \textsc{Feedback Vertex Set} parameterized by degreewidth. We show the former is fixed parameter tractable whereas the latter is NP-hard on sparse tournaments. Additionally, we study \textsc{Feedback Arc Set} on sparse tournaments.

==> complexite_first_draft.tex <==
\section{Computation complexity}
\prob{\BTSAT}
{a CNF formula $\varphi$ where each clause contains exactly three unique literals and each variable occurs two times positively and two time negatively.}
{is there an assignment $\beta$ that satisfies $\varphi$? }

\begin{construction}
  \label{const:3sat}
  Let $\varphi$ be a \BTSAT formula with $m'$ clauses $C_1,\dots,C_{m'}$ clauses and $n'$ variables $x_1,\dots,x_{n'}$. Let $W=n'^3+m'^3$ be an integer. We construct a tournament $T$ as follows.
  \begin{itemize}
    \item Create a regular tournament $A$ of order $W+4\binom{n'}{2}+m'$.
    \item Create two regular tournaments $B$ and $C$ of order $W$ such that $A$ dominates $B\cup C$ and $B$ dominates $C$.
    \item Create a regular tournament $X = \{v_1,v'_1,\dots,v_{n'},v'_{n'}\}$ of order $2n'$ that contains every arc in $\{(v_i,v'_i) \mid i \leq n'\}$ and such that $A\cup C$ dominates $X$ and $X$ dominates $B$. 
    \item Create a sparse tournament $Y$ of order $m'$ with topological ordering $(q_1,\dots,q_{m'})$ such that $A \cup B$ dominates $Y$ and $Y$ dominates $C$.
    \item For each clause $c_{\ell}$ and each variable $x_i$ of $\varphi$,
    \begin{itemize}
      \item if $x_1$ occurs positively in $c_{\ell}$, introduce the arcs $(v_i,q_\ell)$ and $(v'_i,q_\ell)$,
      \item if $x_i$ occurs negatively in $c_\ell$, introduce the arcs $(v_i,q_\ell)$ and $(q_\ell,v'_i)$,
      \item if $x_i$ does not occur in $c_\ell$, introduce the arcs $(v_i,q_\ell)$ and $(q_\ell,v'_i)$.
    \end{itemize}
    \item For each pair of variables $x_i$ and $x_j$, introduce a sparse tournament $U_{i,j} = \{u^{i,j}_1,\bar{u}^{i,j}_1,\dots,u^{i,j}_4,\bar{u}^{i,j}_4,\}$ of order eight such that $U_{i,j}$ dominates $A\cup Y \cup C$, $B$ dominates $U_{i,j}$ and for all pair $(i',j')$ lexicographically smaller than $(i,j)$, $U_{i,j}$ dominates $U_{i',j'}$.  We denote $U = \bigcup_{i,j\leq n'} U_{i,j}$. Moreover, introduce the following paths:
    \begin{itemize}
      \item for all variable $x_k \not\in \{x_i,x_j\}$ and all $t\leq 4$, introduce the paths $(v_k,u^{i,j}_t,v'_k)$ and $(v'_k,\bar{u}^{i,j}_t,v_k)$,
      \item introduce the paths $(v_i,u^{i,j}_1,v'_i)$, $(v_i,\bar{u}^{i,j}_1,v'_i)$, $(v_j,u^{i,j}_1,v'_j)$, $(v_j,\bar{u}^{i,j}_1,v'_j)$,
      \item introduce the paths $(v_i,u^{i,j}_2,v'_i)$, $(v_i,\bar{u}^{i,j}_2,v'_i)$, $(v'_j,u^{i,j}_2,v_j)$, $(v'_j,\bar{u}^{i,j}_2,v_j)$,
      \item introduce the paths $(v'_i,u^{i,j}_3,v_i)$, $(v'_i,\bar{u}^{i,j}_3,v_i)$, $(v_j,u^{i,j}_3,v'_j)$, $(v_j,\bar{u}^{i,j}_3,v'_j)$, and
      \item introduce the paths $(v'_i,u^{i,j}_4,v_i)$, $(v'_i,\bar{u}^{i,j}_4,v_i)$, $(v'_j,u^{i,j}_4,v_j)$, $(v'_j,\bar{u}^{i,j}_4,v_j)$.
\todo{C'est moche}

    \end{itemize}
    \item Introduce a vertex $t$ such that $A\cup C$ dominates $t$ and $t$ dominates $X \cup Y \cup B \cup U$
    \item Finally, introduce two vertex set $H=\{h_1,h_2\}$ with the arc $(h_1,h_2)$ and such that $A \cup B \cup C \cup X \cup Y \cup \{t\}$ dominates $H$ and $H$ dominates $U$.
  \end{itemize}
\end{construction}

We call a vertex of $X$ a \emph{variable vertex} and a vertex of $Y$ a \emph{clause vertex}.

\begin{definition}
  Let $T$ be a tournament resulting from \Cref{const:3sat}. An ordering $\sigma$ of $T$ is \emph{nice} if:
  \begin{itemize}
    \item $A \infor t \infor B \infor U \infor Y \infor C \infor H$, and
    \item for any variable $x_i$, either $t \infor v_i \infor v'_i \infor B$ or $C \infor v_i \infor v'_i \infor H$.
  \end{itemize}
\end{definition}

\input{figure_reduction}
An example of a nice ordering is depicted in \Cref{fig:nice}. Let $\sigma$ be a nice ordering, we call the interval between the vertices of $A$ and the vertices of $B$, the \emph{true zone} and the interval after the vertices of $C$ the \emph{false zone}. Let $q_{\ell}$ be a clause vertex and let $(v_i,v'_i)$ be a pair of variable vertices such that $x_i$ occurs positively (resp. negatively) in $c_\ell$ in $\varphi$. We say that the pair $(v_i,v'_i)$ satisfies $q_\ell$ if $v_i$ and $v'_i$ belong both to the true zone (resp. false zone). Note that there is no backward arc between $q_\ell$ and $\{v_i,v'_i\}$ if and only if $(v_i,v'_i)$ satisfies $q_\ell$. Notice that for any pair of variable vertices $(v_j,v'_j)$ such that $x_i$ does not appear in $q_\ell$, there is exactly one backward arc between $q_\ell$ and $\{v_j,v'_j\}$.

\begin{lemma}
  \label{lemme:nice}
Let $T$ be a tournament resulting from \Cref{const:3sat} and let $\sigma$ be a nice ordering of $T$, we have $\dw(T) \leq W + 4\binom{n'}{2}+ m'+n'+3$. Moreover, for any vertex $w \in V\setminus Y$, we have $\de(w)<W + 4\binom{n'}{2}+ m'+n'+3$.
\end{lemma}

\begin{proof}
  % A
  Let $a$ be a vertex of $A$. Since $A$ is a regular tournament, there are at most $\frac{|A|}{2}= \nicefrac{W}{2}+2\binom{n'}{2}+\nicefrac{m'}{2}$ backward arcs between $a$ and $A \setminus \{a\}$. By construction, there are $|U \cup Y|=8\binom{n'}{2}+m'$ backward arcs between $a$ and $V\setminus A$. Thus, we have $\de(a)\geq \nicefrac{W}{2}+10 \binom{n'}{2} + \nicefrac{3m'}{2}$ and since $W = n'^3+m'^3$, $\de(a) \leq W + 4\binom{n'}{2}+ m'+n'+3$.
%B
  Let $b$ be a vertex of $B$, since $B$ is a regular tournament, there are at most $\frac{|B|}{2}=\nicefrac{W}{2}$ bacward arcs between $b$ and $B \setminus \{b\}$. By construction, there are at most $|X|=2n'$ backward arcs between $b$ and $V\setminus B$. Thus, we have $\de(b)\leq \nicefrac{W}{2} +2n' \leq W + 4\binom{n'}{2}+ m'+n'+3$.
%C
  Let $c$ be a vertex of $C$, since $C$ is a regular tournament, there are at most $\frac{|C|}{2}=\nicefrac{W}{2}$ bacward arcs between $c$ and $C \setminus \{c\}$. By construction, there are at most $|X|=2n'$ backward arcs between $c$ and $V\setminus C$. Thus, we have $\de(c)\leq \nicefrac{W}{2} +2n' \leq W + 4\binom{n'}{2}+ m'+n'+3$. By construction, we have $\de(t)=|C|=W \leq W + 4\binom{n'}{2}+ m'+n'+3$.
%X
  Let $v$ be a vertex of $X$ such that $v \in \{v_i,v'_i\}$ for some variable $x_i$ of $\varphi$. Since $X$ is a regular tournament, there are at most $\nicefrac{|X|}{2}=n'$ backward arcs between $v$ an $X \setminus \{v\}$. If $v$ belongs to the true zone, then there are $|C|=W$ backward arcs between $v$ and $C$ and none between $v$ and $B$. If $v$ belongs to the false zone, then there are $|B|=W$ backward arcs between $v$ and $B$ and none between $v$ and $C$. By construction there are $\frac{|U|}{2}=4\binom{n'}{2}+\nicefrac{m'}{2}$ backward arcs between $v$ and $V\setminus X \cup B \cup C$. Moreover, the number of  backward arcs between $v$ and $Y$ is at most $|Y|=m'$. Thus, we have $\de(v)\leq W + 4\binom{n'}{2}+m' + n'$.
%U
  Let $u$ be a vertex of $U$. There are $|H|=2$ backward arcs between $u$ and $H$. There are $|A| = W + 4 \binom{n'}{2} + m'$ backward arcs between $u$ and $|A|$. Let $(v_i,v'_i)$ be a pair of variable vertices, since $v_i \infor v'_i \infor u$ or $u \infor v_i \infor v'_i$, by construction there is exactly one backward arc between $u$ and $\{v_i,v'_i\}$. Thus, there are $\frac{|X|}{2}=n'$ backward arcs between $u$ and $|X|$. Hence, $\de(u) = W + 4 \binom{n'}{2}+m'+n'+2$.
%H
  Let $h$ be a vertex of $H$. There are $|U|=8\binom{n'}{2}$ backward arcs between $h$ and $U$ and none between $h$ and $V\setminus U$. Thus, we have $\de(h)=8\binom{n'}{2} \leq \dw(T) \leq W + 4\binom{n'}{2}+ m'+n'+3$.
%Y
  Finally, let $q_\ell$ be a vertex of $Y$. By construction, there are $|A|=W+4 \binom{n'}{2} + m'$ backward arcs between $q$ and $A$. Let $v_i$ and $v'_i$ be a pair variable vertices in $X$. If $x_i$ occurs in $c_\ell$, then there are at most two backward arcs between $q_\ell$ and $\{v_i,v'_i\}$. If $x_i$ does not occur in $c_\ell$, then there is one backward arc between $q_\ell$ and $\{v_i,v'_i\}$. Thus, there are at most $n'+3$ backward arcs between $q_\ell$ and $X$. Hence, we have $\de(q_\ell)\leq =W+4 \binom{n'}{2} + m' + n' +3$.
\end{proof}

\begin{lemma}
  \label{lemma:always nice}
Let $T$ be a tournament resulting from \Cref{const:3sat} and let $\sigma$ be an ordering of $T$. There is a nice ordering $\sigma'$ of $T$ such that $\dw[\sigma'](T)\leq \dw(T)$.
\end{lemma}

\begin{proof}
  Let $\sigma$ be an ordering of $T$. If $\dw(T)> W + 4\binom{n'}{2}+ m'+n'+3$, then by \Cref{lemme:nice}, for any nice ordering $\sigma'$ of $T$ we have $\dw[\sigma'](T)<\dw(T)$. Thus, we can suppose that $\dw(T)\leq W + 4\binom{n'}{2}+ m' + n' +3$. We show that it is possible to construct an ordering $\sigma'$ with $\dw[\sigma'](T)\leq \dw(T)$ and having the following properties:
  \begin{enumerate}
    \item $B\infor C$,
    \item $A\infor B$,
    \item $B\infor U \infor Y\infor C$,
    \item $A\infor X$,
    \item $A\infor t\infor B$,
    \item $C\infor H$,
    \item for any vertex $v_i\in X$, either $ v_i \infor  v'_i \infor  B$  or $C\infor v_i\infor v'_i$.
  \end{enumerate}

  \begin{enumerate}
    \item Toward a contradiction, suppose that it exists two vertices $b\in B$ and $c\in C$, such that $c\infor b$. If there is no variable vertex between $c$ and $b$, then we can exchange the positions of $c$ and $b$ in $\sigma$ without increasing the degreewidth of $\sigma$. Suppose that there is a variable vertex $v \in X$ such that $c\infor v\infor b$. Let $B_L = \{b \mid b \in B \wedge b \infor v\}, C_L=\{c \mid c \in C \wedge c \infor v\},B_R=B \setminus B_L$ and $C_R = C \setminus C_L$. (\textit{i.e.} vertices of $B$ and $C$ are partitioned according to whether they are positionned to the left or right of $v$ in $\sigma$). By construction, $\de(v) \geq |B_L| + |C_R|$, thus
    \begin{eqnarray*}
      |B_L|+|C_R| &\leq& W + 4\binom{n'}{2}+ m'+n'+3\\
      2W - |B_R|-|C_L| &\leq& W + 4\binom{n'}{2}+ m' + n' +3\\
      |B_R|+|C_L| &\geq& W - 4\binom{n'}{2} -m'-n'-3.\\
    \end{eqnarray*}
    Suppose that $|C_L| \geq |B_R|$, we have $|C_L|\geq \frac{W-4\binom{n'}{2}-m'-n'-3}{2}$. Consider two cases.
    \begin{enumerate}[(a)]
      \item Suppose it exists a vertex $w\in U \cup Y$ such that $v \infor w$. Let $A_L = \{a \mid a \in A \wedge a \infor w\}$ and $A_R = A \setminus A_L$. Since $\de(w)\geq |C_L|+|A_L|$, we have:
      \begin{eqnarray*}
        |C_L|+|A_L|&\leq& W+ 4\binom{n'}{2}+m'+n'+3\\
        \frac{W-m'-n'-3}{2}-2\binom{n'}{2}+W+4\binom{n'}{2}+m'-|A_R|&\leq& W + 4\binom{n'}{2}+m'+n'+3.\\
        |A_R|&\geq& \frac{W-m'-3n'-9}{2}-2\binom{n'}{2}.\\
      \end{eqnarray*}
      Moreove, we have:
      \begin{eqnarray*}
        \de(v)&\geq& |B_R|+|C_L|+|A_R|\\
        \de(v)&\geq& \frac{3W-3m'-5n'-15}{2}-6\binom{n'}{2}.\\
      \end{eqnarray*}
      Since $W = n'^3+m'^3$, it implies $\de(v)>W+4\binom{n'}{2}+m'+n'+3$ which is a contradiction.
      \item Suppose that $U \cup Y \infor v$. By construction, the number of backward arcs between $v$ and $U \cup Y$ is equal to $\frac{|U\cup Y|}{2} = 4\binom{n'}{2}+\nicefrac{m'}{2}$. Thus, we have $deg(v)\geq |B_L|+|C_R|+4\binom{n'}{2}+\nicefrac{m'}{2}$ which implies:
      \begin{eqnarray*}
        |B_L|+|C_R|+4\binom{n'}{2}+\frac{m'}{2}&\leq& W + 4\binom{n'}{2}+m'+n'+3\\
        2W-|B_R|-|C_L|&\leq& W + \frac{m'}{2}+n' +3\\
        |B_R|+|C_L| &\geq& W -\frac{m'}{2}- n' -3.\\
      \end{eqnarray*}
      Hence, we have $|C_L|\geq \frac{W-\nicefrac{m'}{2}-n'-3}{2}$. Let $b'$ be the rightmost vertex of $B$ in $\sigma$. Since $B$ is a regular tournament, there are $\nicefrac{W}{2}$ backward arcs between $b$ and $B\setminus\{b'\}$. Moreover, the number of backward arcs between $b'$ and $U \cup Y$ is equal to $8\binom{n'}{2}+m'$, by construction. Thus, we have:
      \begin{eqnarray*}
        \de(b')&\geq& |C_L| + \nicefrac{W}{2}+8\binom{n'}{2}+m'\\
        \de(b')&\geq& W + 8\binom{n'}{2}+\frac{3m'}{4} - \frac{n'-3}{2}.\\
      \end{eqnarray*}
      And since $4\binom{n'}{2} \geq \frac{m'}{4}+\frac{3n'+9}{2}$, we have $\de(b')> W +4\binom{n'}{2}+ m'+n'+3$ which is a contradiction.
    \end{enumerate}
    In any case, we reach a contradiction. Samewise, by symmetry, we can use the same arguments to show that the case $|C_L|\geq |B_R|$ leads to a contradiction. Hence, we have $B \infor C$.
    \item Toward a contradiction, suppose that it exists two vertices $a\in A$ and $b \in B$ such that $b\infor a$. If there is no vertex of $U \cup Y$ between $b$ and $a$, then we can exchange the positions of $b$ and $a$ in $\sigma$ without increasing the degreewidth. Hence, we can suppose that there is a vertex $w \in U \cup Y$ such that $b \infor w \infor a$. Let $A_L= \{a' \mid a' \in A \wedge a' \infor w\}, B_L = \{b' \mid b' \in B, b \infor w\},A_R = A \setminus A_L$ and $B\setminus B_L$ (\textit{i.e.} vertices of $B$ and $C$ are partioned according to whether they are positionned to the left or the right of $w$). Let $a'$ be the rightmost vertex of $A$, since $A$ is a regular tournament there are exactly $\frac{W}{2}+2\binom{n'}{2}+\frac{m'}{2}$ backward arcs between $a'$ and $A\setminus \{a'\}$. We have $\de(a') \geq |B_L| + \frac{W+m'}{2} + 2\binom{n'}{2}$ which implies:
    \begin{eqnarray*}
      |B_L| + \frac{W+m'}{2}+2\binom{n'}{2} &\leq& W +4\binom{n'}{2}+ m'+n'+3\\
      W - |B_R| &\leq& \frac{W+m'}{2} + 2\binom{n'}{2} + n' +3\\
      |B_R| &\geq& \frac{W-m'}{2}-2\binom{n'}{2}- n' -3.
    \end{eqnarray*}
    Moreover, since $\de(w)\geq |A_L|+|B_R|$, we have:
    \begin{eqnarray*}
      |A_L|+|B_R| &\leq& W +4\binom{n'}{2}+m'+n' + 3\\
      W + 4\binom{n'}{2}+ m' - |A_R| + |B_R| & \leq & W +4\binom{n'}{2}+ m' + n' +3\\
      |A_R| & \geq& |B_R| - n' - 3 \\
      |A_R| & \geq & \frac{W-m'}{2} -4\binom{n'}{2}-2n'-6.\\
    \end{eqnarray*}
    Now, consider the vertex $t$. If $t \infor C$, then we have $\de(t) \geq |C|+|A_R| > W + m'+n'+3$ which is a contradiction. Thus, there is at least one vertex of $C$ at the left of $t$ in $\sigma$. Since, $B \infor C$, that means $B \infor t$. Let $C_L = \{c' \mid c' \in C \wedge c' \infor t \}$ and $C_R = C \setminus C_L$. We have $\de(t) \geq |B| + |C_R|$. Hence,
\begin{eqnarray*}
  |B| + |C_R| & \leq & W + 4\binom{n'}{2} +m'+n' + 3\\
  2W -|C_L| & \leq &  W + 4\binom{n'}{2} + m'+n' + 3\\
  |C_L| & \leq & W - 4\binom{n'}{2} -m'-n' -3.\\
\end{eqnarray*}
 There is no vertex $w' \in U \cup Y$ such that $t \infor w'$ since otherwise $\de(w') \geq |C_L| + |A| > W + m'+n'+3$. Thus, we have $\de(t) \geq |U\cup Y| + |B| \geq W + 4\binom{n'}{2}+ m' + n' +3$ which is a contradiction. Hence, we have $A \infor B$.
    \item Toward a contradiction, suppose that there are two vertices $w \in U \cup Y$ and $b \in B$ such that $w \infor b$. If there is no variable vertex between $w$ and $b$ in $\sigma$, we can exchange the positions of $b$ and $w$ in $\sigma$ without increasing the degreewidth. Suppose it exists a variable vertex $v$ such that $w \infor v \infor b$ and let $B_L = \{b' \mid b' \in C \wedge b' \infor w\}$ and $B_R = B \setminus B_L$. We have $\de(w) \geq |A|+|B_R|$. Hence,
\begin{eqnarray*}
  |A| + |B_R| & \leq & W + 4\binom{n'}{2} + m' + n' +3\\
  2W + 4\binom{n'}{2} +m' - |B_L| & \leq & W + 4\binom{n'}{2} + m' + n' +3\\
  |B_R| &\geq & W -n' -3.\\
\end{eqnarray*}
    Further, we have $\de(v) \geq |C| + |B_L| > W + m' + n' +3$ which is a contradiction. Thus, we have $B \infor U \cup Y$. By symmetry, we can show that $U \cup Y \infor C$, using the same arguments. Finally, since by construction $U \cup Y$ is a sparse tournament, we can order the vertices of $U \cup Y$ so that $U \infor Y$.
    \item If there are two vertices $a \in A$ and $v \in X$ such that $v \infor a$, then by previous items, there is no clause vertex between $v$ and $a$ in $\sigma$. Thus, we can intervert the positions of $a$ and $v$ in $\sigma$ without increasing the degreewidth. That is, we can obtain an order $\sigma'$ with $A \infor X$.
    \item If there is a vertex $a \in A$ such that $t \infor a$, then by previous items, there is no vertex $w\in U \cup Y$ between $t$ and $a$ in $\sigma$. Thus, we can intervert the positions of $a$ and $t$ in $\sigma$ without increasing the degreewidth. If there is a vertex $b \in B$ such that $b \infor t$, then we can also intervert the positions of $b$ and $t$ in $\sigma$ without increasing the degreewidth. That is, we can obtain an order $\sigma'$ with $A\infor t \infor B$.
    \item First, we show that for any vertex $v \in X$, we have either $v \infor B$ or $C \infor v$ (\textit{i.e.} $v$ is either in the true zone or the false zone). We can not have $B \infor v \infor C$ since otherwise we would have $\de(v) \geq |B|+|C|>2W$. If it exists a vertex $b \in B$ such that $b \infor v \infor C$, then any vertex between $b$ and $v$ in $\sigma$ is a variable vertex or a vertex of $B$ and thus we can exchange the positions of $b$ and $v$ without increasing the degreewidth. If it exists a vertex $c \in C$ such that $B \infor v \infor c$, then any vertex between $c$ and $v$ in $\sigma$ is a variable vertex or a vertex of $C$ and thus we can exchange the positions of $b$ and $v$ without increasing the degreewidth. Further, we show that for every pair $v_i$ and $v'_i$ of variable vertices, we have $v_i \infor v'_i \infor B$ or $C \infor v_i \infor v'_i$. Note that if $v'_i\infor v_i \infor B$ or $C \infor v'_i \infor v_i$, then we can exchange the positions of $v_i$ and $v'_i$ without increasing the degreewidth.
    Let $v_i$ and $v'_i$ be a pair of variable vertices, we say that $(v_i,v'_i)$ is split if $v_i\infor B$ and $C \infor v'_i$ or if $v'_i\infor B$ and $C \infor v_i$ (\textit{i.e.} if $v_i$ and $v'_i$ are not in the same zone).  Recall that number of backward arc between any vertex $u\in U$ and $V\setminus X$ is $|A|+|H|=W+\binom{n'}{2}+m'+2$. Toward a contradiction let $S$ be the set of split pairs. If $|S|=1$, then let $(v_i,v'_i) \in S$ If $v_i \infor v'_i$, then let $u^{j,k}_1$ be a vertex of $U$ such that $j\neq i$ and $k\neq i$. For any pair of variable vertices  $(v_{i'},v'_{i'})\not\in S$, there is exactly one backward arc between $u^{k,j}_1$ and $\{v_{i'},v'_{i'}\}$. Moreover, by construction, there are two backward arcs between $u^{k,j}_1$ and $\{v_{i},v'_{i}\}$, and thus $\de(u^{j,k}_1)=W+\binom{n'}{2}+m'+n'+4$ which is a contradiction. If $v'_i \infor v_i$, we can show the same way that $\de(u^{j,k}_1)=W+\binom{n'}{2}+m'+n'+4$. Hence, $|S|\geq 2$. Let $(v_i,v'_i)$ and $(v_j,v'_j)$ be two pairs of $S$ and consider $U^{i,j}$. By construction, it exists $k\leq 4$ such that there are four backward arcs between $u^{i,j}_k$ and $\{v_i,v'_i,v_j,v'_j\}$ and four backward arcs between $\bar{u}^{i,j}_k$ and $\{v_i,v'_i,v_j,v'_j\}$. Let $S' = \{(v_k,v'_k) \mid v_k \infor v'_k\} \cap S \setminus \{(v_i,v'_i),(v_j,v'_j)\}$ and $S'' = \{(v_k,v'_k) \mid v'_k \infor v_k\} \cap S \setminus \{(v_i,v'_i),(v_j,v'_j)\}$. By construction, the number of backward arcs between $u^{i,j}_k$ and each pair of $S'$ is equal to two and the number of backward arcs between $u^{i,j}_k$ and each pair of $S''$ is equal to zero. Likewise,  the number of backward arcs between $\bar{u}^{i,j}_k$ and each pair of $S''$ is equal to two and the number of backward arcs between $\bar{u}^{i,j}_k$ and each pair of $S'$ is equal to zero. Thus, we have either $\de(u^{i,j}_k)\geq W+\binom{n'}{2}+m'+n'+4$ or $\de(\bar{u}^{i,j}_k)\geq W+\binom{n'}{2}+m'+n'+4$ which is a contradiction. Hence $S$ is empty, that is, for each pair of variable vertices $v_i$ and $v'_i$, we have $v_i\infor v'_i \infor B$ or $C \infor v_i\infor v'_i$.
  \end{enumerate}
\end{proof}

Now we can show the main result of this section.

\begin{theorem}
\DGW is NP-complete
\end{theorem}

\begin{proof}
  Let $\varphi$ be an instance of \BTSAT and $T$ its tournament resulting from \Cref{const:3sat}. We show that $\varphi$ is satisfiable if and only if it exists an ordering $\sigma$ of $T$ such that $\dw(T)<W+4 \binom{n'}{2} + m' +3$.
  \begin{itemize}
    \item[``$\Rightarrow$''] Let $\beta$ be a satisfying assignment for $\varphi$. We construct a nice ordering $\sigma$ of $T$ as follows. For each variable $x_i$, if $\beta(x_i)=\texttt{true}$ then put $v_i$ and $v'_i$ in the true zone. Otherwise, put $v_i$ and $v'_i$ in the false zone. By \Cref{lemme:nice}, for any vertex $w\not\in Y$, we have $\de(w)<W+4 \binom{n'}{2} + m'+n' +3$. Further, let $q_\ell$ be a clause vertex. The number of backward arcs between $q_\ell$ and $V\setminus X$ is equal to $|A|$. Moreover, for every variable $x_i$ that does not occur in $c_\ell$, there is exactly one backward arc between $\{v_i,v'_i\}$ and $q_\ell$. For every variable $x_i \in c_\ell$, if the value of $x_i$ in $\beta$ satisfies $c_\ell$, then there is no backward arc between $\{v_i,v'_i\}$ and $q_\ell$, otherwise there are two backward arcs between $\{v_i,v'_i\}$ and $q_\ell$. Thus, since there is at least one variable in $c_\ell$ that satisfies $c_\ell$, we have $\de(q_\ell)\leq W+4 \binom{n'}{2} + m'+n' +1$. Hence, $\dw(T)<W+4 \binom{n'}{2} + m'+n' +3$.
    \item[``$\Leftarrow$''] Let $\sigma$ be an ordering of $T$ such that $\dw(T)<W+4 \binom{n'}{2} + m'+n' +3$. By \Cref{lemma:always nice}, we can suppose that $\sigma$ is nice. We construct an assignment $\beta$ for $\varphi$ as follows. For each variable $x_i$, if $v_i$ and $v'_i$ are in the true zone, then we set $x_i$ to true. Otherwise, if $v_i$ and $v'_i$ are in the false zone, then we set set $x_i$ to false. Let $c_\ell$ be a variable of $\varphi$. Since $\de(q_\ell)<\dw(T)<W+4 \binom{n'}{2} + m'+n' +3$, there is at least one pair of variable vertices $v_i$ and $v'_i$ such that there is no backward arcs between $\{v_i,v'_i\}$ and $q_\ell$. Thus, by construction, $x_i$ satisfies $c_\ell$. Hence, $\beta$ is a satisfying assignment for $\varphi$.
  \end{itemize}
\end{proof}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> complexityO.tex <==
\section{Computation complexity}
\prob{\BTSAT}
{a CNF formula $\varphi$ where each clause contains exactly three unique literals and each variable occurs two times positively and two time negatively.}
{is there an assignment $\beta$ that satisfies $\varphi$? }
\medskip

Let $\varphi$ be a \BTSAT formula with $m'$ clauses $C_1,\dots,C_{m'}$ clauses and $n'$ variables $x_1,\dots,x_{n'}$.
Since regular tournaments require an odd number of vertices, we have to ensure that $\varphi$ contains an even number of clauses and an odd number of variables. Note that if this is not the case, we can duplicate the formula $\varphi$, and add the three dummy variables $d_1$, $d_2$, $d_3$ and the four following trivial clauses: $d_1 \vee d_2 \vee d_3$, $d_1 \vee \bar{d_2} \vee \bar{d_3}$, $\bar{d_1} \vee d_2 \vee \bar{d_3}$, and $\bar{d_1} \vee \bar{d_2} \vee d_3$.

\begin{construction}
  \label{const:3sat}
  Let $\varphi$ be a \BTSAT formula with $m'$ clauses $C_1,\dots,C_{m'}$ clauses and $n'$ variables $x_1,\dots,x_{n'}$ such that $n'$ is odd and $m'$ is even. Let $W=n'^3+m'^3$ be an odd integer. We construct a tournament $T$ as follows.
  \begin{itemize}
    \item Create a regular tournament $A$ of order $W+2m'+2n'$.
    \item Create two regular tournaments $B$ and $C$ of order $W$ such that $A$ dominates $B\cup C$ and $B$ dominates $C$.
    \item Create an acyclic tournament $X$ of odern $2n'$  with topological ordering $(v_1,v'_1,\dots,v_{n'},v'_{n'})$ such that $A\cup C$ dominates $X$ and $X$ dominates $B$. %\todo[inline]{add extra vertex in $X$}
    \item Create an acyclic tournament $Y$ of order $2m'$ with topological ordering $(q_1,q'_1,\dots,q_{m'},q'_{m'})$ such that $A \cup B$ dominates $Y$ and $Y$ dominates $C$.
    \item For each clause $c_{\ell}$ and each variable $x_i$ of $\varphi$,
    \begin{itemize}
      \item if $x_1$ occurs positively in $c_{\ell}$, then $\{v_i,v'_i\}$ dominates $\{q_\ell,q'_\ell\}$,
      \item if $x_i$ occurs negatively in $c_\ell$, then $\{q_\ell,q'_\ell\}$ dominates $\{v_i,v'_i\}$,
      \item if $x_i$ does not occur in $c_\ell$, then introduce the paths $(v_i,q_\ell,v'_i)$ and $(v'_i,q'_\ell,v_i)$.
    \end{itemize}
    \item Introduce an acyclic tournament $U = \{u^i_p, \bar{u}^i_p \mid i\leq n', p \leq 2\}$ of order $4n'$ such that $U$ dominates $A\cup Y \cup C$ and $B$ dominates $U$. For each variable $x_i$, introduce the following paths:
    \begin{itemize}
      \item for all variable $x_j\neq x_i$ and all $p\leq 2$, introduce the paths $(v_k,u^i_p,v'_k)$ and $(v'_k,\bar{u}^i_p,v_k)$,
      \item introduce the paths $(v_i,u^i_1,v'_i)$, $(v'_i,u^i_2,v_i)$, $(v_i,\bar{u}^i_1,v'_i)$ and $(v'_i,\bar{u}^i_1,v_i)$.
    \end{itemize}
    \item Introduce a vertex $t$ such that $A\cup C $ dominates $t$ and $t$ dominates $X \cup B \cup U \cup Y$
    \item Finally, introduce the two vertices $H=\{h_1,h_2\}$ with the arc $(h_1,h_2)$ and such that $B \cup C \cup X \cup Y \cup \{t\}$ dominates $H$ and $H$ dominates $A \cup U$.
  \end{itemize}
\end{construction}

We call a vertex of $X$ a \emph{variable vertex} and a vertex of $Y$ a \emph{clause vertex}.

\begin{definition}
  Let $T$ be a tournament resulting from \Cref{const:3sat}. An ordering $\sigma$ of $T$ is \emph{nice} if:
  \begin{itemize}
    \item $\sigma$ respects \Cref{lemma:rotational_tournament} property for $A,B$ and $C$,
    \item $A \infor t \infor B \infor U \infor Y \infor C \infor H$, and
    \item for any variable $x_i$, either $t \infor v_i \infor v'_i \infor B$ or $C \infor v_i \infor v'_i \infor H$.
%    \todo[inline]{A,B,U,C,H all have ``good ordering'' (i.e. topological ordering for acyclic tournaments and the ordering described in Lemma~\ref{lemma:rotational_tournament})}
  \end{itemize}
\end{definition}
 
%\input{figure_reduction}
\begin{figure}
	\centering
	\includegraphics[width=0.95\linewidth]{nice_ordering}
	\caption{\label{fig:nice}Example of a nice ordering. A rectangle represent an acyclic tournament, while a rectangle with rounded corners represents a regular tournament. A ``big'' arrow between two intervals $I$ and $I'$ represents the fact that there is a backward between every pair of vertices $i \in I$ and $i' \in I'$. 
		%In this example, we depict one clause vertex $q_1$ and four pairs of variables vertices $\{(v_1,v'_1),\dots,(v_4,v'_4)\}$. In the boolean formula, we have $c_1 = x_1 \vee \neg x_2 \vee x_4$. We can observe that in the depicted ordering, the pairs $(v_1,v'_1)$ and $(v_4,v'_4)$ satisfy $q_1$ whereas the pair $(v_2,v'_2)$ does not.
	}
\end{figure}


An example of a nice ordering is depicted in \Cref{fig:nice}. Let $\sigma$ be a nice ordering, we call the interval between the vertices of $A$ and the vertices of $B$, the \emph{true zone} and the interval after the vertices of $C$ the \emph{false zone}. Let $q_{\ell}$ be a clause vertex and let $(v_i,v'_i)$ be a pair of variable vertices such that $x_i$ occurs positively (resp. negatively) in $c_\ell$ in $\varphi$. We say that the pair $(v_i,v'_i)$ satisfies $q_\ell$ if $v_i$ and $v'_i$ belong both to the true zone (resp. false zone). Note that there is no backward arc between $q_\ell$ and $\{v_i,v'_i\}$ if and only if $(v_i,v'_i)$ satisfies $q_\ell$. Notice that for any pair of variable vertices $(v_j,v'_j)$ such that $x_i$ does not appear in $q_\ell$, there is exactly one backward arc between $q_\ell$ and $\{v_j,v'_j\}$.

\begin{lemma}
  \label{lemme:nice}
Let $T$ be a tournament resulting from \Cref{const:3sat} and let $\sigma$ be a nice ordering of $T$, we have $\dw(T) \leq W + 2m'+3n'+3$. Moreover, for any vertex $w \in V\setminus Y$, we have $\de(w)<W + 2m'+3n'+3$.
\end{lemma}

\begin{proof}
  % A
  Let $a$ be a vertex of $A$. Since $A$ is a regular tournament, there are at most $\frac{|A|}{2}= \frac{W+2m'+2n'}{2}$ backward arcs between $a$ and $A \setminus \{a\}$. By construction, there are $|U \cup Y|=4n'+2m'$ backward arcs between $a$ and $V\setminus A$. Thus, we have $\de(a)\leq \frac{W+6m'+10n'}{2}< W + 2m'+3n'+3$.
%B
  Let $b$ be a vertex of $B$, since $B$ is a regular tournament, there are at most $\frac{|B|}{2}=\frac{W}{2}$ bacward arcs between $b$ and $B \setminus \{b\}$. By construction, there are at most $|X|=2n'$ backward arcs between $b$ and $V\setminus B$. Thus, we have $\de(b)\leq \frac{W}{2} +2n' < W + 2m'+3n'+3$.
%C
  Let $c$ be a vertex of $C$, since $C$ is a regular tournament, there are at most $\frac{|C|}{2}=\frac{W}{2}$ bacward arcs between $c$ and $C \setminus \{c\}$. By construction, there are at most $|X|=2n'$ backward arcs between $c$ and $V\setminus C$. Thus, we have $\de(c)\leq \frac{W}{2} +2n' < W + 2m'+3n'+3$.
%t
  By construction, we have $\de(t)=|C|=W < W + 2m'+3n'+3$.
%X
  Let $v$ be a vertex of $X$ such that $v \in \{v_i,v'_i\}$ for some variable $x_i$ of $\varphi$. There are at most $|X|=2n'$ backward arcs between $v$ and $X \setminus \{v\}$. If $v$ belongs to the true zone, then there are $|C|=W$ backward arcs between $v$ and $C$ and none between $v$ and $B$. If $v$ belongs to the false zone, then there are $|B|=W$ backward arcs between $v$ and $B$ and none between $v$ and $C$. By construction there are $\frac{|U|}{2}=2n'$ backward arcs between $v$ and $U$. Let $Y_i = \{q_\ell,q'_\ell \mid x_i \in c_\ell\}$, if $x_i$ occurs in the clause $c_\ell$, then there is $2$ backward arcs between $v$ and $\{q_\ell,q'_\ell\}$ and none otherwise. Since $x_i$ occurs exactly two times positively and two times negatively, there are $\frac{|Y_i|}{2}$ backward arcs between $v$ and $Y_i$. Moreover, by construction, there are exactly $\frac{|Y\setminus Y_i|}{2}$ between $v$ and $Y \setminus Y_i$. The number of backward arcs between $v$ and $Y$ is $\frac{|Y|}{2}+2=m'$. Thus, we have $\de(v)\leq W +m' + 4n'$. Since $n'<m'$, $\de(v)< W +2m' + 3n'+3$.
%U
  Let $u$ be a vertex of $U$. There are $|H|=2$ backward arcs between $u$ and $H$. There are $|A| = W  + 2m'+2n'$ backward arcs between $u$ and $|A|$. Let $(v_i,v'_i)$ be a pair of variable vertices, since $v_i \infor v'_i \infor u$ or $u \infor v_i \infor v'_i$, by construction there is exactly one backward arc between $u$ and $\{v_i,v'_i\}$. Thus, there are $\frac{|X|}{2}=n'$ backward arcs between $u$ and $|X|$. Hence, $\de(u) = W +2m'+3n'+2$.
%H
  Let $h$ be a vertex of $H$. There are $|U|=4n'$ backward arcs between $h$ and $U$ and none between $h$ and $V\setminus U$. Thus, we have $\de(h)=4n' \leq \dw(T) < W + 2m'+3n'+3$.
%Y
  Finally, let $q_\ell$ be a vertex of $Y$. By construction, there are $|A|=W + 2m' +2n'$ backward arcs between $q$ and $A$. Let $v_i$ and $v'_i$ be a pair variable vertices in $X$. If $x_i$ occurs in $c_\ell$, then there are at most two backward arcs between $q_\ell$ and $\{v_i,v'_i\}$. If $x_i$ does not occur in $c_\ell$, then there is one backward arc between $q_\ell$ and $\{v_i,v'_i\}$. Thus, there are at most $n'+3$ backward arcs between $q_\ell$ and $X$. Hence, we have $\de(q_\ell)\leq =W + 2m' + 3n' +3$.
\end{proof}

\begin{lemma}
  \label{lemma:always nice}
Let $T$ be a tournament resulting from \Cref{const:3sat} and let $\sigma$ be an ordering of $T$. There is a nice ordering $\sigma'$ of $T$ such that $\dw[\sigma'](T)\leq \dw(T)$.
\end{lemma}


\begin{proof}
  Let $\sigma$ be an ordering of $T$. First, if $\dw(T)\geq W + 2m'+3n'+3$, then by \Cref{lemme:nice}, for any nice ordering $\sigma'$ of $T$ we have $\dw[\sigma'](T)\leq\dw(T)$. Thus, we can suppose that $\dw(T)< W + 2m' + 3n' +3$. Second, if $\sigma$ does not respect \Cref{lemma:rotational_tournament} property for $A,B$ or $C$, then we can rearrange the vertices of this tournament to respect these properties. Hence, we can suppose that $\sigma$ respects the property of \Cref{lemma:rotational_tournament}. Further, we show that it is possible to construct an ordering $\sigma'$ with $\dw[\sigma'](T)\leq \dw(T)$ and having the following properties:
  \begin{enumerate}
    \item $B\infor C$,
    \item $A\infor B$,
    \item $B\infor U \infor Y\infor C$,
    \item $A\infor X$,
    \item $A\infor t\infor B$,
    \item $C\infor H$,
    \item for any vertex $v_i\in X$, either $ v_i \infor  v'_i \infor  B$  or $C\infor v_i\infor v'_i$.
  \end{enumerate}

  \begin{enumerate}
    \item Toward a contradiction, suppose that it exists two vertices $b\in B$ and $c\in C$, such that $c\infor b$. If there is no vertex $z \in \{t\}\cup X$ between $c$ and $b$, then we can exchange the positions of $c$ and $b$ in $\sigma$ without increasing the degreewidth of $\sigma$. Suppose that there is a variable vertex $v \in X$ such that $c\infor v\infor b$. Let $B_L = \{b \mid b \in B \wedge b \infor z\}, C_L=\{c \mid c \in C \wedge c \infor z\},B_R=B \setminus B_L$ and $C_R = C \setminus C_L$. (\textit{i.e.} vertices of $B$ and $C$ are partitioned according to whether they are positionned to the left or right of $z$ in $\sigma$). By construction, $\de(z) \geq |B_L| + |C_R|$, thus
    \begin{eqnarray*}
      |B_L|+|C_R| &\leq& W + 2m'+3n'+3\\
      2W - |B_R|-|C_L| &\leq& W +  2m' + 3n' +3\\
      |B_R|+|C_L| &\geq& W -2m'-3n'-3.\\
    \end{eqnarray*}
    We now consider four cases.
    \begin{enumerate}[(a)]
      \item Suppose $|C_L|\geq |B_R|$. We have $|C_L| \geq \frac{W-2m'-3n'-3}{2}$. We handle two different possibilities.
      \begin{enumerate}[({a}1)]
        \item Suppose there is a vertex $w \in U \cup Y$ such that $z\infor w$. Let $A_L = \{a \mid a \in A \wedge a \infor w\}$ and $A_R = A \setminus A_L$. Since $\de(w)\geq |C_L|+|A_L|$, we have:
      \begin{eqnarray*}
        |C_L|+|A_L|&\leq& W+2m'+3n'+3\\
        \frac{W-2m'-3n'-3}{2}+W+2m'+2n'-|A_R|&\leq& W +2m'+3n'+3\\
        |A_R|&\geq& \frac{W-2m'-7n'-9}{2}.\\
      \end{eqnarray*}
      If $|B_R| > \frac{W}{2}$, then let $c'$ be the leftmost vertex of $C$.
      Since $c' \infor z$, we have
      \begin{eqnarray*}
        \de(c')&\geq& \frac{|C|}{2} + |A_R| + |B_R|\\
        \de(c') &>& W + 2m' +3n' +3.\\
      \end{eqnarray*}
      If $|B_R| \leq \frac{W}{2}$, then let $a'$ be the rightmost vertex of $A$.
      Since $A_R$ is not empty, we have $z \infor a$ and thus,
      \begin{eqnarray*}
        \de(a') & \geq & \frac{|A|}{2}+|B_L| + |C_L|\\
        \de(a') & > &W + 2m' +3n' +3.\\
      \end{eqnarray*}
        In any case, we reach a contradiction.
        \item Suppose $U \cup Y \infor z$. By construction, the number of backward arcs between $z$ and $U\cup Y$ is at least $\frac{|U\cup Y|}{2} = m'+2n'$. Thus, we have
        \begin{eqnarray*}
          |B_L| + |C_R| + m' + 2n' & \leq & W + 2m' + 3n' +3\\
          2W - |B_R|-|C_L| &\leq& W + m' + n' + 3 \\
          |B_R| + |C_L| & \geq & W - m'-n'-3.
        \end{eqnarray*}
        Let $b'$ be the rightmost vertex of $B$. Since $B$ is a regular tournament, we have $\frac{|B|}{2}$ backward arcs between $b'$ and $B \setminus \{b'\}$. Moreover, we have $|C_L|$ bacward arcs between $b'$ and $C_L$ and since $U\cup Y \infor z \infor b$, we have $|U \cup Y|$ backward arcs between $b'$ and $U \cup Y$, by construction. Thus, we have:
        \begin{eqnarray*}
          \de(b') & \geq & \frac{|B|}{2} + |C_L| + |U \cup Y| \\
          \de(b') & \geq & \frac{W}{2} + \frac{W-m'-3n'-3}{2} + 2m'+4n' \\
          \de(b') & \geq & W + \frac{3m' + 7n'-3}{2}.
        \end{eqnarray*}
        Since $4n' = 3m'$, we have $\de(b') > W + 2m' + 3n' +3$ which is a contradiction.
      \end{enumerate}
      \item  Suppose $|C_L|< |B_R|$. We have $|B_L| > \frac{W-2m'-3n'-3}{2}$. Again, we handle two different possibilities.
      \begin{enumerate}[({b}1)]
        \item  Suppose there is a vertex $w\in U \cup Y$ such that $w \infor z$. Let $A_L = \{a \mid a \in A \wedge a \infor w\}$ and $A_R = A \setminus A_L$. Since $\de(w) \geq |B_R| + |A_L|$, we have
      \begin{eqnarray*}
        |B_R| + |A_L| & \leq & W + m' +3n'+3\\
        \frac{W-2m'-3n'-3}{2}+W+2m'+2n'-|A_R|&\leq& W +2m'+3n'+3\\
        |A_R|&\geq& \frac{W-2m'-7n'-9}{2}.\\
      \end{eqnarray*}
      If $|C_L|>\frac{W}{2}$, then let $a'$ be the rightmost vertex of $A$. Since $A_R$ is not empty, we have $z \infor a$ and thus,
      \begin{eqnarray*}
        \de(a') & \geq & \frac{|A|}{2}+|B_L| + |C_L|\\
        \de(a') & > &W + 2m' +3n' +3.\\
      \end{eqnarray*}
      If $|C_L|\leq \frac{W}{2}$, then let $c'$ be the leftmost vertex of $C$. Since $c' \infor z$, we have
       \begin{eqnarray*}
        \de(c')&\geq& \frac{|C|}{2} + |A_R| + |B_R|\\
        \de(c') &>& W + 2m' +3n' +3.\\
       \end{eqnarray*}
        In any case, we reach a contradiction.
        % \item Suppose $z \infor U \cup Y$  By construction, the number of backward arcs between $z$ and $U \cup Y$ is equal to $\frac{|U \cup Y|}{2}$. Thus, we have
        % \begin{eqnarray*}
        %   |B_L| + |C_R| + \frac{m'}{2} + 2n' & \leq & W + m' + 3n' + 3\\
        %   2W - |B_R|-|C_L| & \leq & W + \frac{m'}{2}+n'+3\\
        %   |B_R| + |C_L| & \geq & W - \frac{m'}{2} - n' -3.\\
        % \end{eqnarray*}
        % Let $c'$ be the leftmost vertex of $C$. Since $C$ is a regular tournament, we have $\frac{|C|}{2}$ backward arcs between $c'$ and $C\setminus \{c'\}$. Moreover, we have $|B_R|$ backward arcs between $c'$ and $B_R$ and since $c \infor z \infor U \cup Y$, we have $|U \cup Y$ backward arcs between $c'$ and $U \cup Y$, by construction. Thus, we have
        % \begin{eqnarray*}
        %   \de(c') & \geq & \frac{|C|}{2} + |B_R| + |U \cup Y| \\
        %   \de(c') & \geq & \frac{W}{2}+ \frac{W-\nicefrac{m'}{2}- 3n' -3}{2} + m' +4n'\\
        %   \de(c') & \geq & W + \frac{3m'}{4} + \frac{7n'-3}{2}.\\
        % \end{eqnarray*}
        % Since $4n' = 3m'$, we have $\de(b') > W + m' + 3n' +3$ which is a contradiction.
        \item Suppose that $z \infor U \cup Y$. Let $w \in U \cup Y$ and let $A_L = \{a \mid a \in A \wedge a \infor w\}$ and $A_R = A \setminus A_L$. Since $C_L \infor z \infor w$, we have $\de(w) \geq |C_L| + |A_L|$ and thus,
        \begin{eqnarray*}
          |A_L| + |C_L| & \leq & W + 2m' + 3n' +3\\
          2W+2m'+2n' - |A_R| - |C_R| & \leq & W + 2m' +3n' +3\\
%          - |A_R| - |C_R| & \leq & -W  +n' +3\\
          |A_R| + |C_R| & \geq & W  -n' -3\\
          |A_R| & \geq & W  -n' -3 - |C_R|.\\ 
        \end{eqnarray*}
        Since $z \infor w \infor A_R$, by construction we have $\de(z) \geq |B_L| + |C_R| + |A_R|$. Hence,
        \begin{eqnarray*}
          |B_L| + |C_R| + |A_R| & \leq & W + 2m' + 3n' +3 \\
          |B_L| + |C_R| + W -n' -3 - |C_R| & \leq & W + 2m' + 3n' +3\\
          |B_L| & \leq & 2m' + 4n' + 6\\
          |B_R| & \geq & W - 2m' - 4n' - 6.\\
        \end{eqnarray*}
        Let $c'$ be the leftmost vertex of $C$ in $\sigma$. Since $c' \infor z$, we have
        \begin{eqnarray*}
          \de(c') & \geq &\frac{|C|}{2} + |B_R| \\
          \de(c') & \geq &\frac{3W-4m'-8n'-12}{2}.\\
        \end{eqnarray*}
        Since $W = m'^3 + n'^3$, we have $\de(c') > W + 2m' + 3n' + 3$ which is a contradiction.
      \end{enumerate}

    \end{enumerate}
    In any case, we reach a contradiction. Hence, we have $B \infor C$.
    \item Toward a contradiction, suppose that it exists two vertices $a\in A$ and $b \in B$ such that $b\infor a$. If there is no vertex of $U \cup Y$ between $b$ and $a$, then we can exchange the positions of $b$ and $a$ in $\sigma$ without increasing the degreewidth. Hence, we can suppose that there is a vertex $w \in U \cup Y$ such that $b \infor w \infor a$. Let $A_L= \{a' \mid a' \in A \wedge a' \infor w\}, B_L = \{b' \mid b' \in B, b \infor w\},A_R = A \setminus A_L$ and $B\setminus B_L$ (\textit{i.e.} vertices of $B$ and $C$ are partioned according to whether they are positionned to the left or the right of $w$). Let $a'$ be the rightmost vertex of $A$, since $A$ is a regular tournament there are exactly $\frac{W}{2}+m'+n'$ backward arcs between $a'$ and $A\setminus \{a'\}$. We have $\de(a') \geq |B_L| + \frac{W}{2} +m'+n'$ which implies:
    \begin{eqnarray*}
      |B_L| + \frac{W}{2}+m'+n' &\leq& W + 2m'+3n'+3\\
      W - |B_R| &\leq& \frac{W}{2}+ m' + 2n' +3\\
      |B_R| &\geq& \frac{W}{2}-m'-2n' -3.
    \end{eqnarray*}
    Moreover, since $\de(w)\geq |A_L|+|B_R|$, we have:
    \begin{eqnarray*}
      |A_L|+|B_R| &\leq& W +2m'+3n' + 3\\
      W + 2m'+2n' - |A_R| + |B_R| & \leq & W + 2m' + 3n' +3\\
      |A_R| & \geq& |B_R| - n' - 3 \\
      |A_R| & \geq & \frac{W}{2}-m' -3n'-6.\\
    \end{eqnarray*}
    Now, consider the vertex $t$ and consider two cases
    \begin{enumerate}[(a)]
      \item Suppose $t \infor C$. If $t \infor A_R$, then we have $\de(t) \geq |C|+|A_R| > W + 2m'+3n'+3$ which is a contradiction. Otherwise, we have $B_L \infor t$ and then, since $\de(t)\geq |B_L| + |C|$, we have
    \begin{eqnarray*}
      |B_L| + |C| &\leq& W + 2m' + 3n' + 3 \\
      2W-|B_L| &\leq& W + 2m' + 3n' + 3 \\
      |B_R| &\geq & W - 2m' - 3n' -3\\
    \end{eqnarray*}
    Now, consider $a'$ the leftmost vertex of $A$. We have
    \begin{eqnarray*}
      \de(a') &\geq& \frac{|A|}{2} + |B_R| \\
      \de(a') & \geq& \frac{3W-2m'-4n'-6}{2}\\
      \de(a') & >& W+2m'+3n'+3.\\
    \end{eqnarray*}
\item Suppose there is at least one vertex of $C$ at the left of $t$ in $\sigma$. Since, $B \infor C$, that means $B \infor t$. Let $C_L = \{c' \mid c' \in C \wedge c' \infor t \}$ and $C_R = C \setminus C_L$. We have $\de(t) \geq |B| + |C_R|$. Hence,
\begin{eqnarray*}
  |B| + |C_R| & \leq & W  +2m'+3n' + 3\\
  2W -|C_L| & \leq &  W  + 2m'+3n' + 3\\
  |C_L| & \geq & W  -2m'-3n' -3.\\
\end{eqnarray*}
      There is no vertex $w' \in U \cup Y$ such that $t \infor w'$ since otherwise $\de(w') \geq |C_L| + |A| > W + 2m'+3n'+3$. Thus, we have $\de(t) \geq |U\cup Y| + |B| \geq W + 2m' + 3n' +3$ which is a contradiction. 
    \end{enumerate}
    In any case, we reach a contradiction. Hence, we have $A \infor B$.
    \item Toward a contradiction, suppose that there are two vertices $w \in U \cup Y$ and $b' \in B$ such that $w \infor b'$. If there is no variable vertex between $w$ and $b'$ in $\sigma$, we can exchange the positions of $b'$ and $w$ in $\sigma$ without increasing the degreewidth. Suppose it exists a variable vertex $v$ such that $w \infor v \infor b'$ and let $B_L = \{b \mid b \in C \wedge b \infor w\}$ and $B_R = B \setminus B_L$. We have $\de(w) \geq |A|+|B_R|$. Hence,
\begin{eqnarray*}
  |A| + |B_R| & \leq & W + 2m' + 3n' +3\\
  2W  +2m'+2n' - |B_L| & \leq & W +  2m' + 3n' +3\\
  |B_R| &\geq & W -n' -3.\\
\end{eqnarray*}
    Further, we have $\de(v) \geq |C| + |B_L| > W + 2m' + 3n' +3$ which is a contradiction. Thus, we have $B \infor U \cup Y$. By symmetry, we can show that $U \cup Y \infor C$, using the same arguments. Finally, since by construction $U \cup Y$ is an acyclic tournament, we can order the vertices of $U \cup Y$ so that $U \infor Y$.
    \item If there are two vertices $a' \in A$ and $v \in X$ such that $v \infor a'$, then by previous items, there is no clause vertex between $v$ and $a'$ in $\sigma$. Thus, we can intervert the positions of $a'$ and $v$ in $\sigma$ without increasing the degreewidth. That is, we can obtain an order $\sigma'$ with $A \infor X$.
    \item If there is a vertex $a' \in A$ such that $t \infor a'$, then by previous items, there is no vertex $w\in U \cup Y$ between $t$ and $a'$ in $\sigma$. Thus, we can intervert the positions of $a'$ and $t$ in $\sigma$ without increasing the degreewidth. If there is a vertex $b' \in B$ such that $b' \infor t$, then we can also intervert the positions of $b'$ and $t$ in $\sigma$ without increasing the degreewidth. That is, we can obtain an order $\sigma'$ with $A\infor t \infor B$.
    \item Toward a contradiction, suppose that it exists two vertices $h \in H$ and $c \in C$ such that $h \infor c$. If there is no vertex $z \in A \cup U$ between $h$ and $c$, then we can exchange the positions of $z$ and $c$ in $\sigma$ without increasing the degreewidth. If there is a vertex $a \in A$ such that $h \infor a \infor c$, then since $A \infor B$, we have $h \infor B \infor C$. Hence, by construction we have $\de(h) \geq |B|+|C| \geq 2W > W + 2m' + 3n' +3$. If there is a vertex $u \in U$ such that $h \infor u \infor c$, then since $A \infor U \cup C$, we have $A \infor h \infor C$. Hence, by construction we have $\de(h) \geq |A|+|C| \geq 2W + 2m'+2n' > W + 2m' +3n'+3$. In any case, we reach a contradiction and thus, $C \infor H$.
    \item First, we show that for any vertex $v \in X$, we have either $v \infor B$ or $C \infor v$ (\textit{i.e.} $v$ is either in the true zone or the false zone). We can not have $B \infor v \infor C$ since otherwise we would have $\de(v) \geq |B|+|C|\geq 2W>W+2m'+3n'+3$. If it exists a vertex $b' \in B$ such that $b' \infor v \infor C$, then any vertex between $b$ and $v$ in $\sigma$ is a variable vertex or a vertex of $B$ and, we can exchange the positions of $b'$ and $v$ without increasing the degreewidth. If it exists a vertex $c \in C$ such that $B \infor v \infor c$, then any vertex between $c$ and $v$ in $\sigma$ is a variable vertex or a vertex of $C$ and, we can exchange the positions of $b'$ and $v$ without increasing the degreewidth. Further, we show that for every pair $v_i$ and $v'_i$ of variable vertices, we have $v_i \infor v'_i \infor B$ or $C \infor v_i \infor v'_i$. Note that if $v'_i\infor v_i \infor B$ or $C \infor v'_i \infor v_i$, then we can exchange the positions of $v_i$ and $v'_i$ without increasing the degreewidth.
    Let $v_i$ and $v'_i$ be a pair of variable vertices, we say that $(v_i,v'_i)$ is \emph{split} if $v_i\infor B$ and $C \infor v'_i$ or if $v'_i\infor B$ and $C \infor v_i$ (\textit{i.e.} if $v_i$ and $v'_i$ are not in the same zone).  Recall that the number of backward arcs between any vertex $u\in U$ and $V\setminus X$ is $|A|+|H|=W+2m'+2n'+2$. Toward a contradiction let $(v_i,v'_i)$ be a split pair. Suppose that $v_i \infor v'_i$. Then, by construction, there are exactly two backward arcs between $u^i_{2}$ and $\{v_i,v'_i\}$ and two backward arcs between $\bar{u}^i_j$ and $\{v_i,v'_i\}$. Always by construction, for each pair of variable vertices $(v_j,v'_j)$, there is exactly two backward arcs between $\{u^i_2,\bar{u}^i_2\}$ and $\{v_j,v'_j\}$ (either both $u^i_2$ and $\bar{u}^i_2$ are incident to a backward arc if $(v_j,v'_j$) is not split or one of the two vertices is incident to two backward arcs). Suppose without loss of generality that the number of backward arcs between $u^i_2$ and $X \setminus \{v_i,v'_i\}$ is greater or egal to the number of backward arcs between $\bar{u}^i_2$ and $X \setminus \{v_i,v'_i\}$. That is, the number of backward arcs between $u^i_2$ and $X \setminus \{v_i,v'_i\}$ is at least $n'-1$ and thus, the number of backward arcs between $u^i_2$ and $X$ is at least $n'+1$. Hence, $\de(u^i_2)> W+2m'+3n'+3$ which is a contradiction. By symmetry, if $v'_i \infor v_i$, we can show that either $\de(u^i_1)> W+2m'+3n'+3$ or $\de(\bar{u}^i_1)> W+2m'+3n'+3$ which is a contradiction. Hence, no pair of variable vertices is split, that is, for each pair of variable vertices $v_i$ and $v'_i$, we have $v_i\infor v'_i \infor B$ or $C \infor v_i\infor v'_i$.
  \end{enumerate}
\end{proof}

Now we can show the main result of this section.

\begin{theorem}
\DGW is NP-complete
\end{theorem}

\begin{proof}
  Let $\varphi$ be an instance of \BTSAT and $T$ its tournament resulting from \Cref{const:3sat}. We show that $\varphi$ is satisfiable if and only if it exists an ordering $\sigma$ of $T$ such that $\dw(T)<W + 2m' +3n'+3$.
  \begin{itemize}
    \item[``$\Rightarrow$''] Let $\beta$ be a satisfying assignment for $\varphi$. We construct a nice ordering $\sigma$ of $T$ as follows. For each variable $x_i$, if $\beta(x_i)=\texttt{true}$ then put $v_i$ and $v'_i$ in the true zone. Otherwise, put $v_i$ and $v'_i$ in the false zone. By \Cref{lemme:nice}, for any vertex $w\not\in Y$, we have $\de(w)<W+ 2m'+3n' +3$. Further, let $q_\ell$ be a clause vertex. The number of backward arcs between $q_\ell$ and $V\setminus X$ is equal to $|A|$. Moreover, for every variable $x_i$ that does not occur in $c_\ell$, there is exactly one backward arc between $\{v_i,v'_i\}$ and $q_\ell$. For every variable $x_i \in c_\ell$, if the value of $x_i$ in $\beta$ satisfies $c_\ell$, then there is no backward arc between $\{v_i,v'_i\}$ and $q_\ell$, otherwise there are two backward arcs between $\{v_i,v'_i\}$ and $q_\ell$. Thus, since there is at least one variable in $c_\ell$ that satisfies $c_\ell$, we have $\de(q_\ell)\leq W+ 2m'+3n' +1$. Hence, $\dw(T)<W + 2m'+3n' +3$.
    \item[``$\Leftarrow$''] Let $\sigma$ be an ordering of $T$ such that $\dw(T)<W+ 2m'+3n' +3$. By \Cref{lemma:always nice}, we can suppose that $\sigma$ is nice. We construct an assignment $\beta$ for $\varphi$ as follows. For each variable $x_i$, if $v_i$ and $v'_i$ are in the true zone, then we set $x_i$ to true. Otherwise, if $v_i$ and $v'_i$ are in the false zone, then we set $x_i$ to false. Let $c_\ell$ be a variable of $\varphi$. Since $\de(q_\ell)<\dw(T)<W + 2m'+3n' +3$, there is at least one pair of variable vertices $v_i$ and $v'_i$ such that there is no backward arcs between $\{v_i,v'_i\}$ and $q_\ell$. Thus, by construction, $x_i$ satisfies $c_\ell$. Hence, $\beta$ is a satisfying assignment for $\varphi$.
  \end{itemize}
\end{proof}

 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> figure_reduction.tex <==
\begin{figure}[ht]
  \centering 
  \begin{tikzpicture}
    \foreach \a/\b/\c in {-0.5/0.5/gray!25,0.5/1/gray!50,1/4/gray!10,4/5/gray!25,5/6/gray!50,6/9/gray!10,9/10/gray!25,10/13/gray!10,13/14/gray!25}
    \fill [\c] (1.1*\a,0) rectangle (1.1*\b,-2);

    \draw[decorate,decoration={brace,amplitude=1mm}] (-0.5*1.1,0)-- node[midway,above,label=90:{A}] {} (0.5*1.1,0);
    \draw[decorate,decoration={brace,amplitude=1mm}] (0.5*1.1,0)-- node[midway,above,label=90:{$\{t\}$}] {} (1*1.1,0);
    \draw[decorate,decoration={brace,amplitude=1mm}] (4*1.1,0)-- node[midway,above,label=90:{B}] {} (5*1.1,0);
    \draw[decorate,decoration={brace,amplitude=1mm}] (5*1.1,0)-- node[midway,above,label=90:{U}] {} (6*1.1,0);
    \draw[decorate,decoration={brace,amplitude=1mm}] (9*1.1,0)-- node[midway,above,label=90:{C}] {} (10*1.1,0);
    \draw[decorate,decoration={brace,amplitude=1mm}] (13*1.1,0)-- node[midway,above,label=90:{H}] {} (14*1.1,0);

    \draw[decorate,decoration={brace,amplitude=1mm}] (4*1.1,-2)-- node[midway,above,label=-90:{True zone}] {} (1*1.1,-2);
    \draw[decorate,decoration={brace,amplitude=1mm}] (9*1.1,-2)-- node[midway,above,label=-90:{Y}] {} (6*1.1,-2);
    \draw[decorate,decoration={brace,amplitude=1mm}] (13*1.1,-2)-- node[midway,above,label=-90:{False zone}] {} (10*1.1,-2);

    \draw[->] (11.5*1.1,-2.5) to[out=-90,in=-90] (4.5*1.1,-2.5);
    \draw[->] (9.5*1.1,0.75) to[out=90,in=90] (2.5*1.1,0.75);
    \draw[->] (9.5*1.1,0.75) to[out=90,in=90] (0.75*1.1,0.75);
    \draw[->] (7.5*1.1,-2.5) to[out=-90,in=-90] (0,-2.5);

    \foreach[count=\i from 0] \x/\l in {1.5/v_1,2/v'_1,3/v_2,3.5/v'_2,7.5*1.1/q_1,11.6/v_3,12.1/v'_3,13.1/v_4,13.6/v'_4}
    \node[smallvertex,label=90:{$\l$}] (\i) at (\x,-1) {};

    \draw[->] (4) to[bend left] (2);
    \draw[->] (4) to[bend right] (3);
    \draw[->] (5) to[bend right] (4);

  \end{tikzpicture}



  \caption{\label{fig:nice}Example of a nice ordering. A ``big'' arrow between two intervals $I$ and $I'$ represents the fact that there is a backward between every pair of vertices $i \in I$ and $i' \in I'$. In this example, we depict one clause vertex $q_1$ and four pairs of variables vertices $\{(v_1,v'_1),\dots,(v_4,v'_4)\}$. In the boolean formula, we have $c_1 = x_1 \vee \neg x_2 \vee x_4$. We can observe that in the depicted ordering, the pairs $(v_1,v'_1)$ and $(v_4,v'_4)$ satisfy $q_1$ whereas the pair $(v_2,v'_2)$ does not. \todo[inline]{Todo: Update Figure}}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> poly-time_algo.tex <==
\newcommand{\myemph}[1]{{\color{green!40!black}#1}}

\newlength{\RoundedBoxWidth}
\newsavebox{\GrayRoundedBox}
\newenvironment{GrayBox}[1]%
   {\setlength{\RoundedBoxWidth}{.95\textwidth}
    \def\boxheading{#1}
    \begin{lrbox}{\GrayRoundedBox}
       \begin{minipage}{\RoundedBoxWidth}}%
   {   \end{minipage}
    \end{lrbox}
    \begin{center}
    \begin{tikzpicture}%
       \node(Text)[draw=black!20,fill=white,rounded corners,%
             inner sep=2ex,text width=\RoundedBoxWidth]%
             {\usebox{\GrayRoundedBox}};
        \coordinate(x) at (current bounding box.north west);
        \node [draw=white,rectangle,inner sep=3pt,anchor=north west,fill=white] 
        at ($(x)+(6pt,.75em)$) {\boxheading};
    \end{tikzpicture}
    \end{center}}     
            

\section{Polynomial-Time Algorithm}
In this section we design a polynomial time algorithm to decide if a tournament is sparse and if so, then we provide a sparse ordering.
 We call an ordering of a sparse tournament $T$ a \myemph{sparse ordering} if $T$ is sparse with respect to it.
 That is, given a tournament $T=(V,A)$, in time polynomial in $|V|$, we find a linear ordering $\sigma$ of $V$ such that the number of backward arcs incident to a vertex (either as an in-arc or out-arc)  is at most one in the ordering $\sigma$.

\noindent
{\bf Overview.}
The idea is to construct $\sigma$ greedily by iteratively placing a vertex with minimum out-degree as the right-most vertex in $\sigma$ and recursing on smaller sub-tournaments of $T$. A sparse tournament have at least one vertex with out-degree at most one and  \Cref{lemma:low_indegree} guaranties that the set of vertices with out-degree at most one, say $X$, has size at most three. 
 We show that we can correctly identify the ordering of $X$. We delete $X$ from $T$ and recurse on either one or two sub-tournaments of $T$ for $|X| \in\{0,1,3\}$ or $|X|=2$, respectively.
 
Next, we write it formally. We start with two simple observations.
 
 \begin{observation}\label{obs:p-time_min-out-deg}
 Let $T$ be a sparse tournament. Then, there exists a vertex $v$ with $d^+(v) \leq 1$ in $T$.
 \end{observation}
 \begin{proof}
 Suppose not. Then for each $v \in V$, we have that $d^+(v) \geq 2$. Let $T$ is sparse with respect to $\sigma$. Let $v^\star$ be the right-most vertex in $\sigma$.  Then, both the out-neighbors of $v^\star$ are to the left of it in $\sigma$. This is a contradiction to the fact that $T$ is sparse with respect to $\sigma$.
 \end{proof}
 
 \begin{observation}\label{obs:sparse-sub-tournament}
 Let $T'$ be a sub-tournament of $T$. If $T$ is sparse, then so is $T'$.
 \end{observation}
 
 Given a tournament $T$ we produce a sparse ordering $\sigma$ (if exists) as follows. We initialise $\sigma$ to be empty and start constructing it from the right end. For a vertex subset $S$, we write $\langle S\rangle$ to denote an arbitrary ordering of $S$.
 
 \begin{GrayBox}{\textsc{Find-ordering}($T$)}
\begin{enumerate}
\item Let $S = \{v \in V(T) \mid d_T^+(v) =0\}$. 

 if $S \neq \emptyset$, then return $\textsc{Find-ordering}(T[V(T)\setminus S]) \succ \langle S\rangle$.

\item\label{algo:X} Let $X = \{v \in V(T) \mid d_T^+(v) = 1\}$.
\begin{enumerate}
\item if $|X| \in \{ 1,3\}$, then return $\textsc{Find-ordering}(T[V(T)\setminus X]) \succ \langle X\rangle$.

\item\label{algo:X2} if $|X| = 2$, then\\
 let $X=\{x_1,x_2\}$, $(x_2, x_1), (x_1,v) \in A$, for some $v \in V(T) \setminus \{x_1,x_2\}$.
 
 
 \end{enumerate}
\end{enumerate}
$\textsc{Find-ordering}_{vertex}(T,v,X)$
 \begin{enumerate}
 \item if $|N^+(v)| > 2$, then \\
 return
??? 
  $\textsc{Find-ordering}(T[N^-(v) \setminus X]) \succ v \succ \textsc{Find-ordering}(T[N^+(v) \setminus X])~ \succ \textsc{Find-ordering}(T[X]).$
 \item\label{algo:u2} else let $(v,u) \in A$ for some $u \in V(T) \setminus (X \cup \{v\})$.\\
 return 
 ???
 $\textsc{Find-ordering}(T[N^-(u)\setminus\{v\}]) \succ u \succ \textsc{Find-ordering}(T[N^+(u)\setminus \{x_1,x_2\}]) \succ x_1\succ v \succ x_2.$
 \end{enumerate}

\end{GrayBox}% 
 
%\begin{lemma}
%Let $T$ be a sparse tournament and $v \in V$ be a vertex with minimum out-degree in $T$. Then, there exists a sparse ordering $\sigma$ of $T$ with $v$ as the right-most vertex of it.
%\end{lemma} 
\begin{lemma}
The procedure \textsc{Find-ordering}$(T)$ correctly returns a sparse ordering of $T$.
\end{lemma}
\begin{proof}
Let $v \in V(T)$ be a vertex with minimum out-degree in $T$. By \Cref{obs:p-time_min-out-deg}, we have that $d^+(v) \in \{0,1\}$.
\begin{description}
\item[Case 1: $d^+(v) =0$.]\label{item:dv=0} By \Cref{obs:sparse-sub-tournament} $T'= T[V \setminus \{v\}]$ is sparse since $T$ is sparse. Clearly, adding $v$ at the end of the sparse ordering of $T'$ gives a sparse ordering of $T$.

\item[Case 2: $d^+(v) =1$.] Let $X = \{v \in V \mid d^+(v) = 1\}$. By \Cref{lemma:low_indegree}, we have $|X| \leq 3$. Since $d^+(v)$ is $1$, $|X| \geq 1$. We consider different values od $|X|$ seperately. 
\begin{description}
\item If $|X| =1$, then we claim that $v$ is the right-most vertex in each sparse ordering of $T$. 


\item  If $|X| = 3$, then they form a directed triangle and the vertices in $V\setminus X$ are in-neighbors to each vertex in $X$. We put $X$ as the right-most three vertices in some order.
Correctness argument is the same as Case \eqref{item:dv=0}.

\item If $|X| =2$, then let $X=\{x_1, x_2\}$. 
First, observe that either $x_1$ is out-neighbor of $x_2$ or $x_2$ is out-neighbor of $x_1$ as otherwise both cannot have out-degree $1$. 
Without loss of generality, suppose $(x_2, x_1) \in A$. Let the unique vertex in $N^+(x_1) = v$.
We construct an ordering $\sigma$ of $T$ by adding the vertices $x_2, x_1$ in the order at the right end of $\sigma$. We recursively find the sparse orderings $\sigma_1$ and $\sigma_2$ of $T[N^-(v) \setminus X]$ and $T[N^+(v) \setminus X]$, respectively. We claim that $\sigma_1 \succ v \succ \sigma_2 \succ x_2 \succ x_1$ is a sparse ordering of $T$ as described in Step~\eqref{algo:X2}.

We claim the constructed ordering $\sigma$ by our algorithm is a sparse ordering of $T$.
For ease of explanation, we first we consider the case when $d^+(v) >2$. Then, observe that the only possible sparse ordering is $\sigma$.

Otherwise, $d^+(v) = 2$. Note that one of the out-neighbors of $v$ is $x_2$. Let the other out-neighbor be denoted by $u$.  Observer that $x_1$ and $x_2$ are out-neighbors of $u$. 

If $|N^+(u)\setminus X|>1$, then the only possible sparse ordering is as given in the algorithm Step~\eqref{algo:u2}.
Otherwise, let $N^+(u)=\{x_1,x_2,w\}$.  There are only two sparse orderings of $x_1,x_2, v, u$ and $w$, namely, $\pi_1= u \succ w \succ x_1 \succ v \succ x_2$ and $\pi_2= w \succ v \succ u \succ x_2 \succ x_1$. To prove that our algorithm correctly produces a sparse ordering of $T$, we show that if $\sigma^\star$ is a sparse ordering of $T$ with $\sigma^\star$ restricted to $\{x_1,x_2, v, u,w\}$ is $\pi_2$, then $\sigma$ is a sparse ordering of $T$. Note that $\sigma$ restricted to $\{x_1,x_2, v, u,w\}$ is $\pi_1$. 
Observe the following properties of $\sigma^\star$:
\begin{enumerate}
\item $(u,w)$ is a backward arc,
\item $v,u,x_2$ and $x_1$ are consecutive vertices in this order in $\sigma^\star$.
\end{enumerate}
The first point indicates that each vertex in $N^+(w)$ is after $w$ and each vertex in $N^-(w)\setminus\{u\}$ is before $w$ in $\sigma^\star$. Using the second property we have that 
\[\sigma^\star =   \langle N^-(w)\setminus\{u\} \rangle \succ w \succ \langle N^+(w)\setminus \{v,x_1,x_2\} \rangle \succ v \succ u \succ x_2 \succ x_1\]

Since $T$ is sparse with respect to $\sigma^\star$, $N^+(u) = \{x_1,x_2,w\}$, and $N^+(v) = \{u,x_2\}$, then $T$ is sparse with respect to the folowing with backward arcs $(x_2,x_2)$ and $(v,u)$.
\[ \langle N^-(w) \cup \{w\} \cup N^+(w)\setminus \{v,x_1,x_2\} \rangle \succ x_1 \succ v \succ x_2.\]
\end{description} 
\end{description}

\end{proof}

==> regular_tournaments.tex <==
\subsection{Links to other parameters}

\myparagraph{Feedback arc/vertex set} A \textit{feedback arc set} (fas) is a collection of arcs that, when removed from the digraph (or, equivalently, reversed) makes it acyclic. Therefore, it is common to consider the size of the minimal fas as a measure if the digraph is far from being acyclic. In this context, degreewidth comes as a promising alternative. Finding a small subset of arcs hitting all substructures (in this case, directed cycles) of a digraph is one of the fundamental problems in graph theory.
Minimum fas and its vertex-version fvs (defined later) have been widely studied, for numerous applications in many fields, such as circuit design~\cite{Johnson75}, or artificial intelligence~\cite{BGNR98, Dechter90}.
\par

\newJ[I would cut this part now since we're not in Introduction anymore and put the proof of Observation 2 instead]{\todo{S:add this part in introduction. It lacks related works now}More specifically on tournaments (the problem is then called \textit{FAST} for {\sc Feedback Arc Set in Tournaments}), the question whether it is difficult to compute a minimum-FAS on this class of digraphs remained opened for over a decade.
	Conjectured NP-complete by Bang-Jensen and Thomassen~\cite{BT92} in 1992, Ailon \textit{et al.}~\cite{ACN08} were the first ones to its NP-hardness under randomized reductions.
	Since then, deterministic reductions were published~\cite{Alon06, CTY07}.
	From the approximability point of view, van Zuylen and Williamson~\cite{ZW09} provided a 2-approximation of FAST, and Kenyon-Mathieu and Schudy~\cite{KS07} a PTAS algorithm.
	On the parameterized-complexity side, Feige~\cite{Feige09} as well as Karpinski and Schudy~\cite{KS10} independently proved a $2^{O(\sqrt{k})} + n^{O(1)}$ running-time algorithm.}

Note that we can easily bound the degreewidth of a tournament by its minimal fas:

\begin{observationrep}
	For any tournament $T$, we have $\DW(T) \leq fas(T)$.
\end{observationrep}
\begin{proof}
	Consider a tournament $T$, and let $\sigma_f$ be an ordering of $T$ for which the backward arcs are exactly the $k$ arcs of a minimal feedback arc set of $T$. Then, for any vertex $v \in V(T)$, we have $\dw[\sigma_f](v) \leq k$. Therefore, $\DW(T) \leq \dw[\sigma_f](T) \leq k$.
\end{proof}

Note however that the opposite is not true; it is possible to construct tournaments with small degreewidth but large fas, see \cref{fig:link_fvs_fas}.\smallskip


\begin{figure}
	\begin{minipage}{.5\textwidth}
		\centering
		\begin{subfigure}{6.5cm}
			\centering\includegraphics[page = 2, width=0.85\linewidth]{./graphics/link_cutwidth}
			\caption{\label{fig:link_fvs_fas}Example of a tournament with degreewidth one but fas (resp. fvs) $\frac{|V(T)|}{3}$.}
		\end{subfigure}
		\begin{subfigure}{6.5cm}
			\centering\includegraphics[page = 4, width=0.85\linewidth]{./graphics/link_cutwidth}
			\vspace{-1em}
			\caption{\label{fig:link_fvs}Example of a tournament $T$ with fvs one ($v_7$) but degreewidth $\frac{|V(T)| - 3}{2}$. The topological ordering of $T - v_7$ is $\langle v_1, v_2, v_3, v_4, v_5, v_6\rangle$.}
		\end{subfigure}
	\end{minipage}%
	\begin{minipage}{.5\textwidth}
		\centering
		\begin{subfigure}{6.5cm}
			\centering\includegraphics[page = 1, width=0.85\linewidth]{./graphics/link_cutwidth}
			\caption{\label{fig:link_cutwidth}Example of a tournament with degreewidth one but cutwidth $\frac{|V(T)| - 1}{2}$. Since the vertices are sorted by increasing in-degrees (values inside the vertices), this is an optimal ordering for the cutwidth.}
		\end{subfigure}
	\end{minipage}%
	\caption{Link between degreewidth and other parameters. All the non-depicted arcs are forward.}
	\label{fig:links_with_parameters}
\end{figure}





Similarly, a \textit{feedback vertex set} (fvs) consists in a collection of vertices that, when removed from the digraph makes it acyclic. However, \--- unlike the feedback arc set \--- the link between feedback vertex set and degreewidth seem less clear; we can easily construct tournaments with low degreewidth and large fvs (see  \cref{fig:link_fvs_fas}) as well as large degreewidth and small fvs (see \cref{fig:link_fvs}). \smallskip



\myparagraph{Cutwidth} Let us first recall the definition of the cutwidth of a digraph. Given an ordering $\sigma:= \langle v_1, \dots, v_n \rangle$ of the vertices of a digraph $D$, we say that a prefix of $\sigma$ is a sequence of consecutive vertices $\langle v_1, \dots, v_k \rangle$ for some $k \in [n]$. We associate for each prefix of $\sigma$ a \textit{cut} defined as the set of backward arcs with head in the prefix and tail outside of it. The \textit{width} of the ordering $\sigma$ is defined as the maximum sized
cut among all the possible prefixes of $\sigma$. Finally, the cutwidth of $D$, denoted $ctw(D)$, is the minimum width among all the orderings of the vertex set of $D$.
It is well-known that computing cutwidth is NP-complete~\cite{gavril1977some}, and has a $O(\log^2(n))$-approximation on general graphs \cite{leighton1999multicommodity}.
When $D$ is a tournament, one can compute an optimal ordering for the cutwidth by sorting the degrees according to the in-degrees~\cite{Fradkin2011}. Note that we will use the same idea to show a 3-approximation algorithm to compute degreewidth in \cref{th:approx}.

Intuitively, the difference between the cutwidth and the degreewidth is that the former focuses on the backward arcs going ``above'' the intervals between the vertices while the latter focuses on the backward arcs coming from and to the vertices themselves.
Observe that for any tournament $T$, the degreewidth is bounded by a function of the cutwidth. Formally, we have the following

\begin{observation}
	For any tournament $T$, we have $\DW(T) \leq 2ctw(T)$.
\end{observation}

\newJ{\begin{proof}
		Consider a tournament $T$, and let $\sigma_c$ be an optimal ordering of $T$ for the cutwidth. Then, let $v$ be a vertex such that $\dw[\sigma_c](v) = \dw[\sigma_c](T)$, the number of backward arcs with $v$ as a tail (resp. with $v$ as a head) cannot be larger than $ctw(T)$ without contradicting the optimality of $\sigma_c$. Therefore, we have $\dw(T) \leq \dw[\sigma_c](T)  = \dw[\sigma_c](v) \leq 2 ctw(T)$.
	\end{proof}
}


Note however that the opposite is not true; it is possible to construct tournaments with small degreewidth but large cutwidth, see \cref{fig:link_cutwidth}.\smallskip



\smallskip




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

